ShanghaiTech at MRP 2019: Sequence-to-Graph Transduction with Second-Order Edge Inference for Cross-Framework Meaning Representation Parsing

This paper presents the system used in our submission to the \textit{CoNLL 2019 shared task: Cross-Framework Meaning Representation Parsing}. Our system is a graph-based parser which combines an extended pointer-generator network that generates nodes and a second-order mean field variational inference module that predicts edges. Our system achieved \nth{1} and \nth{2} place for the DM and PSD frameworks respectively on the in-framework ranks and achieved \nth{3} place for the DM framework on the cross-framework ranks.

==> Makefile <==
.PHONY: clean release

clean:
	rm *.aux *.log *.bbl *.blg *.out *~

release:
	-make clean;
	tar zpScvf ../../public/latex.tgz --transform='s@^@mrp/2019/latex/@'\
	  *



==> data_process.tex <==
\section{Appendix}

We introduce our pre-processing and post-processing in our work for amr parsing, eds parsing and ucca parsing

\subsection{AMR data processing}
Our data processing is following \citet{zhang-etal-2018-stog}. The main difference is that we use lemmas and POS tags from the companion data but not from CoreNLP, and the NER tags are from {\color{blue} xx}. 

In pre-processing, we first get the the lemmas, POS tags and NER tags for input tokens. Then, we remove the senses in amr nodes, and remove the wiki links and polarity attributes. At last, we replace the sub-graphs of special entities, such as names, places, times, with the anonymized word. The corresponding phrases in the sentences are also anonymized. A mapping from NER tags to this entities is build to process the test data.

In post-processing, we generate the AMR sub-graphs from the anonymizations. Then we assign the senses and add wiki links and polarity attributes with the method in \citet{zhang-etal-2018-stog}.

\subsection{EDS and UCCA data processing}
In pre-processing we first clean the companion data to make sure the tokens in companion data is the same as mrp input. Then we get the NER tags from {\color{blue} xx}. We also replace the anchors with the index of start token and end token, as it is easy to predict. 

For UCCA data, we label the empty node(node without 'label') with 'n_"id"', where the "id" is the order that the empty node appears in the node sequence.

For EDS data, we count the long nodes that a node corresponding to a span with more than one token. For a span with more then one tokens, if the probability that it corresponds to a long node (else, it corresponds to several nodes) is more than 0.5 and the long node appears twice or more in the training set, this span is combined into one token. {\color{blue} Other process}.

In post-processing, we compute the anchors from the predicted token indexes. {\color{blue} Other process about eds}.
